Retrieval Enhanced Data Augmentation for Question Answering on Privacy Policies

Prior studies in privacy policies frame the question answering (QA) task as identifying the most relevant text segment or a list of sentences from a policy document given a user query. Existing labeled datasets are heavily imbalanced (only a few relevant segments), limiting the QA performance in this domain. In this paper, we develop a data augmentation framework based on ensembling retriever models that captures the relevant text segments from unlabeled policy documents and expand the positive examples in the training set. In addition, to improve the diversity and quality of the augmented data, we leverage multiple pre-trained language models (LMs) and cascade them with noise reduction filter models. Using our augmented data on the PrivacyQA benchmark, we elevate the existing baseline by a large margin (10\% F1) and achieve a new state-of-the-art F1 score of 50\%. Our ablation studies provide further insights into the effectiveness of our approach.

==> tables/bert_ret_F1_cat.tex <==
\begin{table}[!ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{\hskip 0.05in}l@{\hskip 0.05in}|c|c|c} 
\hline
Opp-115 Category & BERT & PBERT & SimCSE \\ 
% \begin{tabular}{@{\hskip 0.05in}c@{\hskip 0.05in}|@{\hskip 0.05in}c@{\hskip 0.05in}|c@{\hskip 0.1in} c|c@{\hskip 0.1in} c}
% \hline
% \multirowcell{2}{Opp-115 \\ category} & \multirowcell{2}{SQuAD \\ Pre-training}  & \multicolumn{2}{c|}{Valid} & \multicolumn{2}{c}{Test}  \\ 
% \cline{3-6}
% & & EM & F1 & EM & F1 \\ 
\hline\hline
First Party Collection/Use & { 48.33} & {\color{red}{46.14}} & {\color{red}{ 45.71}}\\
Third Party Sharing/Collection & {\color{red}{ 37.81}}  & {\color{red}{ 36.55}} & {39.10} \\  
Data Security & { 62.77} & {60.52} & {\color{red}{ 57.27}} \\  
Data Retention & { 42.87}  & {\color{red}{ 35.33}} & {41.49} \\  
User Access, Edit and Deletion & { 52.47}  & {\color{red}{47.47}} & {\color{red}{41.26}}\\ 
User Choice/Control & {\color{red}{38.91}} & { 58.83} & {\color{red}{36.65}} \\
Other &  { 55.38} & {\color{red}{44.68}} & { 54.29} \\ 
\hline
% Overall & 46.00 & 46.94 & 46.99 \\
% \hline
\end{tabular}
}
\vspace{-2mm}
\caption{Test performance breakdown of BERT-base model for privacy practice categories, sorted by the average answer length as indicated by $|\text{ans}|$.
}
\label{table:per-type-filtered}
% \vspace{-2mm}
\end{table}

==> tables/no_bert_ret_F1_unfilter.tex <==
% \begin{table}[!ht]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{\hskip 0.05in}l@{\hskip 0.05in}|c|c|c} 
% \hline
% Opp-115 Category & BERT & PBERT & SimCSE \\ 
% % \begin{tabular}{@{\hskip 0.05in}c@{\hskip 0.05in}|@{\hskip 0.05in}c@{\hskip 0.05in}|c@{\hskip 0.1in} c|c@{\hskip 0.1in} c}
% % \hline
% % \multirowcell{2}{Opp-115 \\ category} & \multirowcell{2}{SQuAD \\ Pre-training}  & \multicolumn{2}{c|}{Valid} & \multicolumn{2}{c}{Test}  \\ 
% % \cline{3-6}
% % & & EM & F1 & EM & F1 \\ 
% \hline\hline
% First Party Collection/Use & 44.59 & 46.14 & { 46.44}\\
% Third Party Sharing/Collection & { 43.07}  & {36.55} & {41.44} \\  
% Data Security & { 64.87} & {60.52} & 60.43 \\  
% Data Retention & { 52.48}  & { 35.33}  & 34.83 \\  
% User Access, Edit and Deletion & { 71.94}  & 47.47  & 31.23 \\
% User Choice/Control & 41.15 & { 59.83} & 42.26  \\
% Other &  { 36.46} & {{44.68}} & 51.89 \\ 
% \hline
% Overall & 44.70 & 46.94 & 47.77\\
% \hline
% \end{tabular}
% }
% \vspace{-2mm}
% \caption{Test performance breakdown of BERT-base model for privacy practice categories, sorted by the average answer length as indicated by $|\text{ans}|$.
% }
% \label{table:breakdown_result}
% % \vspace{-2mm}
% \end{table}



% \begin{table}[!ht]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{\hskip 0.05in}l@{\hskip 0.05in}|c|c|c|c|c} 
% \hline
% Opp-115 Category & \% & BERT & PBERT & SimCSE & Ours \\ 
% % \begin{tabular}{@{\hskip 0.05in}c@{\hskip 0.05in}|@{\hskip 0.05in}c@{\hskip 0.05in}|c@{\hskip 0.1in} c|c@{\hskip 0.1in} c}
% % \hline
% % \multirowcell{2}{Opp-115 \\ category} & \multirowcell{2}{SQuAD \\ Pre-training}  & \multicolumn{2}{c|}{Valid} & \multicolumn{2}{c}{Test}  \\ 
% % \cline{3-6}
% % & & EM & F1 & EM & F1 \\ 
% \hline\hline
% First Party Collection & 42 & 45 & {\bf 46} & {\bf 46} & \\
% Third Party Sharing & 25 &  {\bf 43}  & {37} & {41} \\ 
% Data Security & 11 & {\bf 65} & {61} & 60 \\  
% Data Retention & 4 & {\bf 52}  & {35}  & 35 \\  
% User Access/Edit & 2 &  {\bf 72}  & 48  & 31 \\
% User Choice/Control & 7 & 41 & {\bf 60} & 42  \\
% Other & 9 &  {36} & {{45}} & {\bf 52} \\ 
% \hline
% Overall & 100 & 45 & 47 & 48 & 50 \\
% \hline
% \end{tabular}
% }
% \vspace{-2mm}
% \caption{Test performance breakdown of BERT-base model for privacy practice categories, sorted by the average answer length as indicated by $|\text{ans}|$.
% }
% \label{table:breakdown_result}
% % \vspace{-2mm}
% \end{table}

\begin{table}[!ht]
% \centering
\hspace{-1.7mm}
\resizebox{1.02\linewidth}{!}{
\begin{tabular}{@{\hskip 0.05in}l@{\hskip 0.05in}|c|c|c|c} 
\hline
Opp-115 Category & \% & PBERT-R & SimCSE-R & \toolextnospace \\ 
% \begin{tabular}{@{\hskip 0.05in}c@{\hskip 0.05in}|@{\hskip 0.05in}c@{\hskip 0.05in}|c@{\hskip 0.1in} c|c@{\hskip 0.1in} c}
% \hline
% \multirowcell{2}{Opp-115 \\ category} & \multirowcell{2}{SQuAD \\ Pre-training}  & \multicolumn{2}{c|}{Valid} & \multicolumn{2}{c}{Test}  \\ 
% \cline{3-6}
% & & EM & F1 & EM & F1 \\ 
\hline\hline
First Party Collection & 42 & {46.14} & {\bf 46.44} & {\color{blue} \bf } \\
Third Party Sharing & 25 & { 43.07}  & {36.55} & {\color{blue} \bf } \\ 
Data Security & 11  & {60.52} & 60.43 &  \\  
Data Retention & 4   & {35}  & 35 & {\color{blue} \bf 56} \\  
User Access/Edit & 2   & 48  & 31 & 61 \\
User Choice/Control & 7  & {\bf 60} & 42 & {\color{red} 31} \\
Other & 9 &  {36}  & {\bf 52} & {\color{blue} \bf 55} \\ 
\hline
Overall & 100 & 47 & 48 & 50 \\
\hline
\end{tabular}
}
\vspace{-2mm}
\caption{Test performance breakdown of different retriever augmented models.
}
\label{table:per-cat-f1}
% \vspace{-2mm}
\end{table}


% \begin{table}[!ht]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{\hskip 0.05in}l@{\hskip 0.05in}|c|c|c} 
% \hline
% Opp-115 Category & BERT & PBERT & SimCSE \\ 
% % \begin{tabular}{@{\hskip 0.05in}c@{\hskip 0.05in}|@{\hskip 0.05in}c@{\hskip 0.05in}|c@{\hskip 0.1in} c|c@{\hskip 0.1in} c}
% % \hline
% % \multirowcell{2}{Opp-115 \\ category} & \multirowcell{2}{SQuAD \\ Pre-training}  & \multicolumn{2}{c|}{Valid} & \multicolumn{2}{c}{Test}  \\ 
% % \cline{3-6}
% % & & EM & F1 & EM & F1 \\ 
% \hline\hline
% First Party Collection/Use & 45 & {\bf 46} & {\bf 46}\\
% Third Party Sharing/Collection & {\bf 43}  & {37} & {41} \\  
% Data Security & {\bf 65} & {61} & 60 \\  
% Data Retention & {\bf 52}  & {35}  & 35 \\  
% User Access, Edit and Deletion & {\bf 72}  & 48  & 31 \\
% User Choice/Control & 41 & {\bf 60} & 42  \\
% Other &  {36} & {{45}} & {\bf 52} \\ 
% \hline
% Overall & 45 & 47 & 48\\
% \hline
% \end{tabular}
% }
% \vspace{-2mm}
% \caption{Test performance breakdown of BERT-base model for privacy practice categories, sorted by the average answer length as indicated by $|\text{ans}|$.
% }
% \label{table:breakdown_result}
% % \vspace{-2mm}
% \end{table}





==> tables/retrieval_examples.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
\centering
% \vspace{4mm}
\resizebox{\linewidth}{!}{%
 \small
\def\arraystretch{1.5}%
\begin{tabular}{p{0.99\linewidth}}
\hline
Q: who all has access to my medical information? \\
\hline
% \medskip
\vspace{-2mm}
% {\bf Gold:} i) Apple HealthKit to health information and to share that information with your healthcare providers. ii) Your use of our Application with that healthcare institution may be subject to that healthcare institution's policies and terms. \\
% \vspace{-6mm}
% \noskip
{\color{blue}\bf Correct retrievals:} 
(S) We may share your information with other health care providers, laboratories, govt. agencies, insurance companies, organ procurement organizations, or medical examiners. 
% -SimCSE-R
% 2) Do not sell your personal or medical information to anyone.
% -BERT-R
(P) Lab, Inc will transmit personal health information to authorized medical providers. 
% PBERT-R
% (R3) To organ and tissue donation requests: By law, we can disclose health information about you to organ procurement organizations.
% -BERT-R
\\
\vspace{-6mm}
{\color{red}\bf Incorrect retrievals:} 
(S) However, we take the protection of your private health information very seriously. 
(P) All doctors, and many other healthcare professionals, are included in our database.
% (R3) You may be able to access your pet’s health records or other information via the Sites.
% iv) will say “yes” unless a law requires us to disclose that health information.
% iv) do not claim that our products “cure” disease.
% ii) Has no access to your database password or any data stored in your local database on your devices.
\\
\hline
\end{tabular}
}
\vspace{-1mm}
\caption{
\small Retrieval examples: S (\emph{SimCSE-R}), P (\emph{PBERT-R}).}
\label{table:ret-example}
\vspace{-2mm}
\end{table}
